Estimation Rates for Sparse Linear Cyclic Causal Models

Causal models are important tools to understand complex phenomena and predict the outcome of controlled experiments, also known as interventions. In this work, we present statistical rates of estimation for linear cyclic causal models under the assumption of homoscedastic Gaussian noise by analyzing both the LLC estimator introduced by Hyttinen, Eberhardt and Hoyer and a novel two-step penalized maximum likelihood estimator. We establish asymptotic near minimax optimality for the maximum likelihood estimator over a class of sparse causal graphs in the case of near-optimally chosen interventions. Moreover, we find evidence for practical advantages of this estimator compared to LLC in synthetic numerical experiments.

==> Arxiv 2019-06-07/commandes.tex <==


\newcommand{\DS}{\displaystyle}
\newcommand{\intbeta}{\lfloor \beta \rfloor}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\sA}{\mathsf{A}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sZ}{\mathsf{Z}}

\newcommand{\hB}{\hat{B}}
\newcommand{\hBi}{\hat{B}_{\mathrm{init}}}
\newcommand{\hT}{\hat{T}}
\newcommand{\hb}{\hat{b}}
\newcommand{\hatt}{\hat{t}}
\newcommand{\init}{\mathrm{init}}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\llc}{\mathrm{llc}}


\newcommand{\bone}{\mathbf{1}}



\newcommand{\R}{{\rm I}\kern-0.18em{\rm R}}
\newcommand{\h}{{\rm I}\kern-0.18em{\rm H}}
\newcommand{\K}{{\rm I}\kern-0.18em{\rm K}}
\newcommand{\p}{{\rm I}\kern-0.18em{\rm P}}
\newcommand{\E}{{\rm I}\kern-0.18em{\rm E}}
\newcommand{\Z}{{\rm Z}\kern-0.18em{\rm Z}}
\newcommand{\1}{{\rm 1}\kern-0.24em{\rm I}}
\newcommand{\N}{{\rm I}\kern-0.18em{\rm N}}

\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\X}{\field{X}}
\newcommand{\Y}{\field{Y}}
\newcommand{\bbS}{\field{S}}
\newcommand{\n}{\mathcal{N}}
\newcommand{\x}{\mathcal{X}}

\newcommand{\qq}{{\sf q}}
\newcommand{\pp}{{\sf p}}
\newcommand{\hh}{{\sf h}}
\newcommand{\ff}{{\sf f}}
\newcommand{\fF}{{\sf F}}
\newcommand{\pP}{{\sf P}}
\newcommand{\qQ}{{\sf Q}}


\newcommand{\phin}{\varphi_n}
\newcommand{\phinb}{\overline \varphi_n(t)}
\newcommand{\pn}{\p_{\kern-0.25em n}}
\newcommand{\pnm}{\p_{\kern-0.25em n,m}}
\newcommand{\psubm}{\p_{\kern-0.25em m}}
\newcommand{\psubp}{\p_{\kern-0.25em p}}
\newcommand{\cfi}{\cF_{\kern-0.25em \infty}}
\newcommand{\ic}{\mathrm{i}}
\newcommand{\symdiff}{%
  \mathbin{\text{\footnotesize$\bigtriangleup$}}}
\newcommand{\symdiffsmall}{%
  \mathbin{\text{\scriptsize $\bigtriangleup$}}}
\newcommand{\Leb}{\mathrm{Leb}_d}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\ddelta}{d_{\symdiffsmall}}
\newcommand{\dsubh}{d_H}
\newcommand{\dsubX}{d_X}

\newcommand{\spann}{\mathop{\mathrm{span}}}
\newcommand{\card}{\mathop{\mathrm{card}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\re}{\mathrm{Re}}
\newcommand{\im}{\mathrm{Im}}
\newcommand{\epr}{\hfill\hbox{\hskip 4pt\vrule width 5pt
                  height 6pt depth 1.5pt}\vspace{0.5cm}\par}

\newcommand{\eps}{\varepsilon}
\newcommand{\Deq}{\stackrel{\mathcal{D}}{=}}

\newcommand{\ubar}{\underbar}
\newcommand{\Kbeta}{K_{\hspace{-0.3mm} \beta}}
%\newcommand{\crzero}{\overset{r_0}{\underset{}{\longleftrightarrow}}}
\newcommand{\crzero}[1]{\overset{r_0}{\underset{#1}{\longleftrightarrow}}}
\newcommand{\ind}{\mathrel{\bot\mskip -8,5mu\bot}}
\newcommand{\bi}{^{(i)}}
\newcommand{\bj}[1]{^{(#1)}}
\newcommand{\spp}{\mathrm{Sp}}

%Theoremes en Anglais
\newtheorem{TH1}{Theorem}[section]
\newtheorem{ex}{Example}[section]
\newtheorem{exo}{Exercise}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{lem}{Lemma}[section]
\newtheorem{rem}{Remark}[section]
\newtheorem{rems}{Remarks}[section]
%\newtheorem{fact}{Fact}
\newtheorem{hyp}{Assumption}
\newtheorem{cond}{Condition}
\newtheorem{defin}{Definition}[section]
%\newcounter{equation}[section]
\renewcommand{\theequation}{\thesection.\arabic{equation}}
%\renewcommand{\tilde}{\widetilde}

%Theoremes en Francais
\newtheorem{TH1fr}{Theor\`eme}[section]
\newtheorem{corfr}{Corollaire}[section]
\newtheorem{exfr}{Exemple}[section]
\newtheorem{exofr}{Exercice}[section]
\newtheorem{propfr}{Proposition}[section]
\newtheorem{lemfr}{Lemme}[section]
\newtheorem{remfr}{Remarque}[section]
\newtheorem{remsfr}{Remarques}[section]
%\newtheorem{factfr}{Fait}
\newtheorem{hypfr}{Hypoth\`ese H \kern-0.24em}
\newtheorem{definfr}{D\'efinition}[section]

%Cadres d'algorithmes
\newlength{\minipagewidth}
\setlength{\minipagewidth}{\textwidth}
\setlength{\fboxsep}{3mm}
\addtolength{\minipagewidth}{-\fboxrule}
\addtolength{\minipagewidth}{-\fboxrule}
\addtolength{\minipagewidth}{-\fboxsep}
\addtolength{\minipagewidth}{-\fboxsep}
\newcommand{\bookbox}[1]{
\par\medskip\noindent
\framebox[\textwidth]{
\begin{minipage}{\minipagewidth}
{#1}
\end{minipage} } \par\medskip }
%

%sauts
\newcommand{\vp}{\vspace{.25cm}}
\newcommand{\vm}{\vspace{.5cm}}
\newcommand{\vg}{\vspace{1cm}}
\newcommand{\vgneg}{\vspace{-1cm}}
\newcommand{\vneg}{\vspace{-.5cm}}
\newcommand{\vpneg}{\vspace{-.25cm}}

%tailles
\newcommand{\tp}{\ptsize{10}}
\newcommand{\douzp}{\ptsize{12}}
\newcommand{\np}{\ptsize{9}}
\newcommand{\hp}{\ptsize{8}}



%Couleurs


\newcommand{\fr}{\selectlanguage{francais}}

\hyphenation{semi--su-per-vis}
\hyphenation{in-d} 
\hyphenation{pen-dant}
\hyphenation{solve--the--equa-tion}

